Memorization in NLP Fine-tuning Methods

Large language models are shown to present privacy risks through memorization of training data, and several recent works have studied such risks for the pre-training phase. Little attention, however, has been given to the fine-tuning phase and it is not well understood how different fine-tuning methods (such as fine-tuning the full model, the model head, and adapter) compare in terms of memorization risk. This presents increasing concern as the "pre-train and fine-tune" paradigm proliferates. In this paper, we empirically study memorization of fine-tuning methods using membership inference and extraction attacks, and show that their susceptibility to attacks is very different. We observe that fine-tuning the head of the model has the highest susceptibility to attacks, whereas fine-tuning smaller adapters appears to be less vulnerable to known extraction attacks.

==> body/related_work.tex <==
\paragraph{Related work.}
Previous work has explored memorization in the pre-training phase of language models and the effect of the addition of out-of-distribution data in the training set. Various attacks have been devised in recent years to explore the level of memorization in these models. In this paper, we focus on membership inference attacks (MIA) and the effect of various fine-tuning methods on memorization in language models.  \dnote{is there a reason to focus on MIA here - we use both exposure and MIA in our experiments. If we are space-limited, I think this who related work section could be cut, just need to make sure we are mentioning the relevant related work where necessary later (or earlier) and avoid duplication}
 
An MIA tries to determine if a target sample was used to train a target model or not \cite{https://doi.org/10.48550/arxiv.1610.05820, https://doi.org/10.48550/arxiv.1709.01604, jayaraman2021revisiting}, whereas, a training data extraction attack quantifies the risk of memorization in language models by probing the trained model \cite{247690, carlini2019secret, 10.1145/3372297.3417880, https://doi.org/10.48550/arxiv.2012.07805, https://doi.org/10.48550/arxiv.2202.07646, https://doi.org/10.48550/arxiv.2101.00036}. The presence of unintended memorization in neural language models can lead to major privacy breaches, which is distinctly shown by \cite{carlini2019secret} and can be quantified through their exposure metric. Additionally, some progress has been made in examining the perturbation in memorization on the exclusion of particular samples from the training data \cite{https://doi.org/10.48550/arxiv.2112.12938}. In this work, we use a recent MIA \cite{mireshghallah2022quantifying}, which makes use of a reference model and a likelihood ratio test to provide a stronger measurement of training data leakage in masked language models, helps us analyze the various fine-tuning methods and the level of data leakage they bring about in language models.\tw{the MIA part is also redundant (repeating what section 4 says). maybe we remove related work completely (merging into sec 3 and 4)?}

\dnote{this paragraph is background, not related work - not sure we need it here, seems redundant with the next section}
In terms of fine-tuning, the work most relevant to ours is adapter tuning~\cite{houlsby2019parameter}, as we experiment with it as a fine-tuning method. Adapters are generally used to fine-tune a model for a new task without revisiting the previous tasks. This helps curb the retraining of the model for every new task. Recent research has also spotlighted prefix tuning \cite{li2021prefix}, an alternative to fine-tuning for natural language generation tasks. Prefix-tuning involves freezing the language model's parameters and optimizing only a small continuous task-specific vector i.e. the prefix prepended to the input. Furthermore, \cite{https://doi.org/10.48550/arxiv.2110.04366} presents a unified framework for the state-of-the-art parameter-efficient transfer learning approaches and demonstrates adapter fine-tuning and prefix tuning are very similar. 

